Identifying public values and spatial conflicts in urban planning

Identifying the diverse and often competing values of citizens, and resolving the consequent public value conflicts, are of significant importance for inclusive and integrated urban development. Scholars have highlighted that relational, value-laden urban space gives rise to many diverse conflicts that vary both spatially and temporally. Although notions of public value conflicts have been conceived in theory, there are very few empirical studies that identify such values and their conflicts in urban space. Building on public value theory and using a case-study mixed-methods approach, this paper proposes a new approach to empirically investigate public value conflicts in urban space. Using unstructured participatory data of 4,528 citizen contributions from a Public Participation Geographic Information Systems in Hamburg, Germany, natural language processing and spatial clustering techniques are used to identify areas of potential value conflicts. Four expert workshops assess and interpret these quantitative findings. Integrating both quantitative and qualitative results, 19 general public values and a total of 9 archetypical conflicts are identified. On the basis of these results, this paper proposes a new conceptual tool of Public Value Spheres that extends the theoretical notion of public-value conflicts and helps to further account for the value-laden nature of urban space.

==> sections/00_formalities.tex <==
\section{Formalities}

\begin{itemize}
    \item \textbf{Word restriction:} Between 4,000 and 8,500 words (including abstract, references, notes, appendices, tables and figures). One table or figure will count as approximately half a page of text or 250 words. If your paper exceeds the specified word limit it will be withdrawn
    \item \textbf{Covering letter:} Authors should explain in their covering letter how their submitted paper engages with broad international debates in urban theory, and should consider how their paper fits with past and ongoing debates in the Urban Studies journal. We strongly encourage authors to familiarise themselves with, and cite where appropriate, articles in the journal relevant to their own perspectives and arguments
    \item \textbf{File Type:} Only electronic files conforming to the journal's guidelines will be accepted. Preferred formats for the text and tables of your manuscript are Word DOC and Excel. Please also refer to additional guideline on submitting artwork below.
    \item \textbf{Referencing:} Urban Studies adheres to the SAGE Harvard reference style
    \item \textbf{Supplemental Files:} This journal is able to host approved supplemental materials online, alongside the full-text of articles. Supplemental files will be subjected to peer-review alongside the article.  For more information please refer to SAGE’s
    \item Manuscripts include an abstract and five keywords
    % \item Usage of ORCID iD is encouraged
    
\end{itemize}


%see: https://www.sagepub.com/sites/default/files/SAGE_UK_style_guide_short.pdf
